TRINIDI: Time-of-Flight Resonance Imaging with Neutrons for Isotopic Density Inference

Accurate reconstruction of 2D and 3D isotope densities is a desired capability with great potential impact in applications such as evaluation and development of next-generation nuclear fuels. Neutron time-of-flight (TOF) resonance imaging offers a potential approach by exploiting the characteristic neutron absorption spectra of each isotope. However, it is a major challenge to compute quantitatively accurate images due to a variety of confounding effects such as severe Poisson noise, background scatter, beam non-uniformity, absorption non-linearity, and extended source pulse duration. We present the TRINIDI algorithm which is based on a two-step process in which we first estimate the neutron flux and background counts, and then reconstruct the areal densities of each isotope and pixel. Both components are based on the inversion of a forward model that accounts for the highly non-linear absorption, energy-dependent emission profile, and Poisson noise, while also modeling the substantial spatio-temporal variation of the background and flux. To do this, we formulate the non-linear inverse problem as two optimization problems that are solved in sequence. We demonstrate on both synthetic and measured data that TRINIDI can reconstruct quantitatively accurate 2D views of isotopic areal density that can then be reconstructed into quantitatively accurate 3D volumes of isotopic volumetric density.

==> versions/submission_2-10-2023/inputs/defs.tex <==

% ---------- Draft definitions --------------------
%\def\draft{} % comment this to turn off abouts

\ifdefined\draft

    \usepackage{marginnote}
    \addtolength\paperwidth{200pt}
    \addtolength\hoffset{100pt}
    \addtolength\marginparwidth{100pt}
    \addtolength\marginparsep{-5pt}
    \addtolength\marginparwidth{82pt}

    
    \newcommand{\about}[1]{\marginnote{\textsf{\color{green}\scriptsize#1}}}
    
\else
    \newcommand{\about}[1]{}
\fi
%  -  -  -  -  -  -  -  -

\ifdefined\draft
    \newcommand{\todo}[1]{\textsf{\color{red}\scriptsize[#1]}}
\else
    \newcommand{\todo}[1]{}

\fi


% -----------------------------------------------



    %\newcommand{\note}[1]{\vspace{-0.6em}\textsf{\textit{\color{blue}\tiny#1}}\vspace{-0.4em}\par}
    %\newcommand{\todo}[1]{\vspace{-0.6em}\textsf{\textit{\color{red}\tiny ToDo: #1}}\vspace{-0.4em}\par}

\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line


\usepackage{wrapfig}
\usepackage{blindtext}
\usepackage{upgreek}

\newcommand{\horrule}[1]{\rule{\linewidth}{#1}} % Create horizontal rule command with 1 argument of height

\renewcommand\ttdefault{cmvtt}



\newcommand{\ie}{i.e.\xspace}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\etal}{et al.\xspace}


\newcommand{\eq}[1]{\eqref{eq:#1}}
\newcommand{\fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\tab}[1]{Table~\ref{tab:#1}}
\newcommand{\figs}[1]{Figures~\ref{fig:#1}}
\newcommand{\fign}[1]{\ref{fig:#1}}
\newcommand{\sctn}[1]{Section~\ref{sec:#1}}
\newcommand{\appx}[1]{Appendix~\ref{app:#1}}



\newcommand{\n}[1]{\mathrm{#1}} % normal roman
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mbs}[1]{\boldsymbol{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\ran}{\mathop{\mathrm{ran}}}
\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\prox}{{\mathrm{prox}}}
\newcommand{\proj}{{\mathrm{proj}}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\del}{\nabla}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\shrink}{shrink}
\DeclareRobustCommand{\orderof}{\ensuremath{\mathcal{O}}}
\newcommand{\imod}{\mathop{\mathrm{mod}}}
\newcommand{\idiv}{\mathop{\mathrm{div}}}



==> versions/submission_2-10-2023/inputs/head.tex <==


\title{TRINIDI: Time-of-Flight Resonance Imaging with Neutrons for Isotopic Density Inference}



\author{
    Thilo Balke,~\IEEEmembership{Student Member,~IEEE},
    Alexander M. Long,
    Sven C. Vogel,
    Brendt Wohlberg,~\IEEEmembership{Fellow,~IEEE},
    Charles A. Bouman,~\IEEEmembership{Fellow,~IEEE} 
    %\thanks{Manuscript received April 19, 2021; revised August 16, 2021.}
    \thanks{
    %\centerline{-------------}
        Thilo Balke and Brendt Wohlberg are with Theoretical Division, Los Alamos National Laboratory, Los Alamos, NM 87545 USA. %, and also with School of Electrical and Computer Engineering, Purdue University, West Lafayette, IN 47907 USA.
        E-mail: \texttt{thilo.balke@gmail.com}, \texttt{brendt@lanl.gov}
    }
    \thanks{
        Alexander M. Long and Sven C. Vogel are with Materials Science and Technology Division, Los Alamos National Laboratory, Los Alamos, NM 87545 USA. E-mail: \texttt{alexlong@lanl.gov}, \texttt{sven@lanl.gov}
    }
    %\thanks{
    %    Brendt Wohlberg is with Theoretical Division, Los Alamos National %Laboratory, Los Alamos, NM 87545 USA. E-mail: \texttt{brendt@lanl.gov}
    %}
    \thanks{
        Charles A. Bouman is with the School of ECE and BME of Purdue University, West Lafayette, IN 47907 USA. E-mail: \texttt{bouman@purdue.edu}
    }
    \thanks{
        Research was supported by the Laboratory Directed Research and Development program of Los Alamos National Laboratory under project number 20200061DR, and partially supported by NSF grant number CCF-1763896.
    }
}



% The paper headers
%\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2021}%
%{Shell \MakeLowercase{\textit{et al.}}: A Sample Article Using IEEEtran.cls for IEEE Journals}

%\IEEEpubid{0000--0000/00\$00.00~\copyright~2021 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.




\maketitle




==> versions/submission_2-10-2023/inputs/notes.tex <==

%--------------------------------
\setcounter{page}{0}
\textbf{EDICS}

\begin{itemize}
    \item \textbf{CIF-OBI}	% Optimization-based Inversion Methods: Surrogate methods; Large-scale methods; Non-linear methods; Proximal iterative methods, Dual-decomposition methods; Convex relaxation; Splitting methods; Alternating direction method of multipliers
    \item \textbf{CIS-SSI}	% Spectral Sensing: Hyperspectral, Spectroscopic, and Remote sensing imaging
    \item \textbf{CIS-TIM}	% Tomographic Imaging: Computed transmission tomography (CT); Single photon emission computed tomography (SPECT); Positron emission tomography (PET); Diffuse optical tomography (DOT); Dose reduction methods; Phase-contrast imaging; Other tomographic imaging
\end{itemize}




\iffalse
    \vspace{1cm}
    \textbf{Name of Algorithm}
    \begin{table}[htb]
        \centering
        \begin{tabular}{ll}
    MAD\textunderscore NEUTRON & MAterial Decomposition NEUTRON\\
    MAD\textunderscore TONI & MAterial Decomposition TOF Neutron Imaging\\
    MAD\textunderscore ERNI & MAterial Decomposition Energy-Resolved Neutron Imaging\\
    ENIGMADEC & Energy-resolved Neutron ImaginG with MAterial DEComposition\\
    MANDI & MAterial Neutron Decomposition Imaging\\
    MADESIN & MAterial DEcomposition through Spectral Imaging with Neutrons\\
    MADELIN & MAterial DEcomposition through Energy-resoLved Imaging with Neutrons\\
    MAD\textunderscore HERNIA & MAterial Decomposition Hyperspectral Energy-Resolved Neutron ImAging\\
    NITRIDR & Neutron Imaging of Time-of-flight Resonances for Isotope Density Reconstruction\\
    NITRIDE & Neutron Imaging of Time-of-flight Resonances for Isotope Density Estimation\\
    TRINIDy & TOF Resonance Imaging with Neutrons for Isopope DensitY / DensitrometrY\\
    TRINIDI & TOF Resonance Imaging with Neutrons for Isopope Density Inference
        \end{tabular}
    \end{table}
\fi

\vspace{1cm}

%\fbox
{\adjincludegraphics[width=0.8\columnwidth,
trim={{0.0\width} {0.0\height} {0.0\width} {0.0\height}}
% trim (left, bottom, right, top)
,clip]{Figure/trinidi.png}}
% trim (left, bottom, right, top)

\vspace{1cm}

\texttt{LA-UR-23-21022}

\todo{ToDo}% When you have a final manuscript accepted by the publisher, return to http://rassti.lanl.gov and upload a PDF of your accepted, peer-reviewed manuscript using the Accepted Manuscripts button.  For more information see http://int.lanl.gov/library/rassti/am.shtml



%--------------------------------


==> versions/submission_2-10-2023/inputs/packages.tex <==
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{array}
\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp}
\usepackage{stfloats}
\usepackage{cuted}
\usepackage{url}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{cite}
\hyphenation{op-tical net-works semi-conduc-tor IEEE-Xplore}
% updated with editorial comments 8/9/2021


\usepackage[export]{adjustbox}
\usepackage{xfrac}  

\usepackage{booktabs}
\usepackage{enumitem}




\usepackage{xcolor}
\usepackage[switch]{lineno}
\usepackage{lipsum}


\usepackage{amssymb}
\usepackage{booktabs}
% \usepackage[bookmarks=false]{hyperref}
\usepackage[bb=boondox]{mathalfa}


\usepackage[english]{babel} % English
% \usepackage{breqn}
\usepackage{cancel}


% \usepackage[toc,page]{appendix}



==> versions/submission_2-10-2023/inputs/tail.tex <==


% \cite{boyd2011distributed}

\bibliographystyle{IEEEbib}
\bibliography{refs}



% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}\vspace{-33pt}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
% Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
% Use the author name as the 3rd argument followed by the biography text.
% \end{IEEEbiography}

% \vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}

%\begin{IEEEbiography
%[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biophoto/balke}}]
%\begin{IEEEbiographynophoto}
%{Thilo\ Balke} (Student Member, IEEE) 
%\end{IEEEbiography}
%\end{IEEEbiographynophoto}

%\begin{IEEEbiography
%[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biophoto/balke}}]
%\begin{IEEEbiographynophoto}
%{Alexander M. Long}
%\end{IEEEbiography}
%\end{IEEEbiographynophoto}


%\begin{IEEEbiography
%[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biophoto/balke}}]
%\begin{IEEEbiographynophoto}
%{Sven C. Vogel} 
%\end{IEEEbiography}
%\end{IEEEbiographynophoto}


%\begin{IEEEbiography
%[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biophoto/wohlberg}}]
%\begin{IEEEbiographynophoto}
%{Brendt\ Wohlberg} (Senior Member, IEEE)
%\end{IEEEbiography}
%\end{IEEEbiographynophoto}

%\begin{IEEEbiography
%[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biophoto/balke}}]
%\begin{IEEEbiographynophoto}
%{Charles A. Bouman} (Fellow, IEEE) 
%\end{IEEEbiography}
%\end{IEEEbiographynophoto}

\vfill

